Multi-Level Feedback Generation with Large Language Models for Empowering Novice Peer Counselors

Realistic practice and tailored feedback are key processes for training peer counselors with clinical skills. However, existing mechanisms of providing feedback largely rely on human supervision. Peer counselors often lack mechanisms to receive detailed feedback from experienced mentors, making it difficult for them to support the large number of people with mental health issues who use peer counseling. Our work aims to leverage large language models to provide contextualized and multi-level feedback to empower peer counselors, especially novices, at scale. To achieve this, we co-design with a group of senior psychotherapy supervisors to develop a multi-level feedback taxonomy, and then construct a publicly available dataset with comprehensive feedback annotations of 400 emotional support conversations. We further design a self-improvement method on top of large language models to enhance the automatic generation of feedback. Via qualitative and quantitative evaluation with domain experts, we demonstrate that our method minimizes the risk of potentially harmful and low-quality feedback generation which is desirable in such high-stakes scenarios.

==> tex/feedback_framework.tex <==

% \begin{table*}[ht]
% \centering
%   \resizebox{\textwidth}{!}{
%   % \begin{tabular}{p{25mm}p{105mm}p{60mm}}
%     \begin{tabular}{p{25mm}p{105mm}p{60mm}}
%     \hline
%     Area & Definition & Support from mental health literature\\
    
%     \hline
%    Structure & This skill assists the counselor and client in guiding the conversation effectively, ensuring productive use of time, and covering essential topics. A basic structure, while flexible to individual needs, provides both parties with a sense of security and direction. 
%    & \cite{day1980structuring, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive} \\
%    Reflections & This skill involves repeating or rephrasing clients' statements to identify and acknowledge their feelings. This technique helps clarify the client's emotions and encourages them to explore these feelings further. &  \cite{bugental2001handbook, rautalinko2007reflective, arnold2014behind, hill2009helping, moyers2014motivational, moyers2016motivational, perez-rosas-etal-2019-makes, beck2020cognitive, shah2022modeling}\\
%    Questions & Questions in peer counseling can be formulated either as inquiries (e.g., "How do you feel about that?") or as prompts (e.g., "Tell me more about your feelings on that"), provided to aid the client in understanding or examining their emotions. & \cite{bugental2001handbook, hill2009helping, james2010science, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Suggestions & This technique involves offering specific directives or advice that clients can apply outside the counseling sessions &  \cite{bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Validation & Validation goes beyond simply acknowledging a client's feelings. It actively affirms their experiences and perspectives as understandable and worthy of respect, even if the counselor may not personally share their viewpoints &  \cite{linehan1997validation, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive}\\
%    Self-disclosure & Sharing of personal experiences can create a sense of empathy and connection, reducing the client's feeling of isolation. This approach is balanced to avoid overshadowing the client's emotions or introducing irrelevant personal details. &  \cite{henretty2010role, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Empathy & This skill involves understanding the client's emotions and sharing in their experience, offering a sense of being truly seen and heard. This deeper connection allows counselors to guide clients toward self-discovery and provide targeted support
% &  \cite{bugental2001handbook, hill2009helping, beck2020cognitive, cooper2020mindfulness, sharma-etal-2020-computational}  \\
%    Professionalism & Professionalism refers to setting clear boundaries and using appropriate language and communication style.& \cite{bugental2001handbook, hill2009helping} \\
%    \hline
   
   
% \end{tabular}
% }
%   \caption{Dimensions of effective helper-communication: key utterance level active listening skills areas. }
%   \label{tab:effective_communication}
% \end{table*}

% \begin{table*}[ht]
% \centering
%   \resizebox{1.1\textwidth}{!}{
%   \begin{tabular}{p{20mm}p{105mm}p{50mm}p{60mm}}
%     \hline
%     Active listening skills & Definition  & Excerpts from the interviews & Support from psychiatry literature\\
    
%     \hline
    
%    Structure & This skill assists the counselor and client in guiding the conversation effectively, ensuring productive use of time, and covering essential topics. A basic structure, while flexible to individual needs, provides both parties with a sense of security and direction. & 
%        \begin{tabular}{c}
%             \\
%        \end{tabular}

%    & \cite{day1980structuring, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive} \\

   
%    Reflections & This skill involves repeating or rephrasing clients' statements to identify and acknowledge their feelings. This technique helps clarify the client's emotions and encourages them to explore these feelings further. & & \cite{bugental2001handbook, rautalinko2007reflective, arnold2014behind, hill2009helping, moyers2014motivational, moyers2016motivational, perez-rosas-etal-2019-makes, beck2020cognitive, shah2022modeling}\\
%    Questions & Questions in peer counseling can be formulated either as inquiries (e.g., "How do you feel about that?") or as prompts (e.g., "Tell me more about your feelings on that"), provided to aid the client in understanding or examining their emotions. & & \cite{bugental2001handbook, hill2009helping, james2010science, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Suggestions & This technique involves offering specific directives or advice that clients can apply outside the counseling sessions & & \cite{bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Validation & Validation goes beyond simply acknowledging a client's feelings. It actively affirms their experiences and perspectives as understandable and worthy of respect, even if the counselor may not personally share their viewpoints & & \cite{linehan1997validation, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive}\\
%    Self-disclosure & Sharing of personal experiences can create a sense of empathy and connection, reducing the client's feeling of isolation. This approach is balanced to avoid overshadowing the client's emotions or introducing irrelevant personal details. & & \cite{henretty2010role, bugental2001handbook, hill2009helping, moyers2014motivational, moyers2016motivational, beck2020cognitive, shah2022modeling}\\
%    Empathy & This skill involves understanding the client's emotions and sharing in their experience, offering a sense of being truly seen and heard. This deeper connection allows counselors to guide clients toward self-discovery and provide targeted support
% & & \cite{bugental2001handbook, hill2009helping, beck2020cognitive, cooper2020mindfulness, sharma-etal-2020-computational}  \\
%    Professionalism & Professionalism refers to setting clear boundaries and using appropriate language and communication style.& & \cite{bugental2001handbook, hill2009helping} \\
   
   
% \end{tabular}
% }
%   \caption{Dimensions of effective helper-communication: key utterance level active listening skills. \raj{To do - add quotes}}
%   \label{tab:effective_communication}
% \end{table*}


% \item[--] \textbf{Reflections} involve repeating or rephrasing clients' statements to identify and acknowledge their feelings. This technique helps clarify the client's emotions and encourages them to explore these feelings further \cite{rautalinko2007reflective, hill2009helping,arnold2014behind}.

% \item[--] \textbf{Questions} in peer-counseling can be formulated either as inquiries (e.g., "How do you feel about that?") or as prompts (e.g., "Tell me more about your feelings on that"), provided with the objective of aiding the client in understanding or examining their emotions \cite{hill2009helping, james2010science}.

% \item[--] \textbf{Suggestions} involve offering specific directives or advice that clients can apply outside the counseling sessions \cite{hill2009helping}.

% \item[--] \textbf{Validation} goes beyond simply acknowledging a client's feelings. It actively affirms their experiences and perspectives as understandable and worthy of respect, even if the counselor may not personally share their viewpoints \cite{linehan1997validation}.

% \item[--] \textbf{Self-disclosure} realized via ethical and strategic sharing of personal experiences can create a sense of empathy and connection, reducing the client's feeling of isolation. This approach is balanced to avoid overshadowing the client's emotions or introducing irrelevant personal details \cite{henretty2010role}.

% \item[--] \textbf{Empathy} involves not only understanding the client's emotions but also sharing in their experience, offering a sense of being truly seen and heard. This deeper connection allows counselors to guide clients toward self-discovery and provide targeted support
% \cite{elliott2018therapist, cooper2020mindfulness, sharma-etal-2020-computational}.

% \item[--] \textbf{Professionalism}
% involves setting clear boundaries and using appropriate language and communication style.

% \item[--] \textbf{Structure} assists the counselor and client in guiding the conversation effectively, ensuring productive use of time and covering essential topics. A basic structure, while flexible to individual needs, provides a sense of security and direction for both parties \cite{day1980structuring}. 

% \end{itemize}
